On the characterization of asymptotic cases of the diffusion equation with rough coefficients and applications to preconditioning

We consider the diffusion equation in the setting of operator theory. In particular, we study the characterization of the limit of the diffusion operator for diffusivities approaching zero on a subdomain $\Omega_1$ of the domain of integration of $\Omega$. We generalize Lions' results to covering the case of diffusivities which are piecewise $C^1$ up to the boundary of $\Omega_1$ and $\Omega_2$, where $\Omega_2 := \Omega \setminus \overline{\Omega}_1$ instead of piecewise constant coefficients. In addition, we extend both Lions' and our previous results by providing the strong convergence of $(A_{\bar{p}_\nu}^{-1})_{\nu \in \mathbb{N}^\ast},$ for a monotonically decreasing sequence of diffusivities $(\bar{p}_\nu )_{\nu \in \mathbb{N}^\ast}$.

==> mathabx.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% mathabx.tex. Version: May 18, 2005.
% Author: Anthony PHAN.
% matches the ``mathabx'' family.
% plain-TeX input file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\ifx\mathabxversion\undefined\else\endinput\fi
\def\mathabxversion{January 28, 2004}%
%
\catcode`@=11
%
% proofing?
%

\ifx\proofmode\undefined
	\def\symbol@message#1{\relax}%
	\def\symbol@mark#1#2{\relax}%
	\def\check@definition#1{\relax}%
	\def\mathabx@undefine#1{\let#1=\undefined}%
	\def\mathabx@aliases#1#2{\@mathabx@aliases#1#2?\@end}
	\def\@mathabx@aliases#1#2#3\@end{\ifx#2?\else
		\let#2=#1\@mathabx@aliases#1#3\@end\fi}%
\else
	\def\symbol@message#1{\vskip\z@ plus\baselineskip
		\penalty-250\vskip\z@ plus-\baselineskip
		\medbreak{\noindent\bf #1}%
		\nobreak\smallskip\noindent\ignorespaces}%
	\def\symbolsp@cing#1{\ifcase\number#1 ord\or op%
		\or bin\or rel\or open\or close\or punct%
		\or var\else other\fi}%
	\def\symbol@mark#1#2{\allowbreak
		\hbox to 0.05\hsize{$#1$\hss}%
		\hbox to 0.05\hsize{\unhbox0\hss}%
		\hbox to 0.4001\hsize{{\tt\string#1}%
		$^{\rm\symbolsp@cing{#2}}$\hfil}%
		\ignorespaces}%
	\def\check@definition#1{\ifx#1\undefined
		\setbox0\hbox{}%
		\else\setbox0=\hbox{$#1\relax$}\fi}%
	\def\mathabx@undefine#1{}%
	\def\mathabx@aliases#1#2{\setbox0=\lastbox
		\@mathabx@aliases#1#2?\@end
		\ifdim\wd0>0.4\hsize\hbox to 0.9001\hsize{\unhbox0\hfill}%
		\else\hbox to 0.4001\hsize{\unhbox0\hfill}\fi}%
	\def\@mathabx@aliases#1#2#3\@end{\ifx#2?\else
		\let#2=#1%
		\setbox0=\hbox{\unhbox0, \tt\string#2}%
		\@mathabx@aliases#1#3\@end\fi}%
\fi
%
% Symbols declarations: \LaTeX-like commands
%
\def\hexnumber@#1{\ifcase\number#1 0\or 1\or 2\or 3\or 4%
	\or 5\or 6\or 7\or 8\or 9\or A\or B\or C\or D\or E\else F\fi}%
\def\hexnumber@@#1{{\count0=#1
	\count1=#1
	\divide\count0 by 16
	\hexnumber@\count0
	\multiply\count0 by 16
	\advance\count1 by -\count0
	\hexnumber@\count1}}%
%
\def\DeclareMathSymbol#1#2#3#4{\check@definition{#1}%
	\count255=#2\multiply\count255 by 16
	\advance\count255 by \csname#3fam\endcsname
	\multiply\count255 by 256\advance\count255 by #4
	\ifcat\noexpand#1\relax\mathchardef#1=\count255%
	\else\expandafter
		\mathcode\expandafter`\csname#1\endcsname=\count255%
	\fi\symbol@mark{#1}{#2}}%
%
\def\gobble@quotes#1{\ifx#1"\else#1\fi}%
%
\def\@DeclareMathDelimiter#1#2#3#4#5#6{%
	\edef#1{\noexpand\delimiter\noexpand"\gobble@quotes#2%
	\expandafter\hexnumber@\csname#3fam\endcsname\gobble@quotes#4%
	\expandafter\hexnumber@\csname#5fam\endcsname\gobble@quotes#6 }%
	\symbol@mark{#1}{#2}}%
%
\def\@xDeclareMathDelimiter#1#2#3#4#5{%
	\count255=\csname#2fam\endcsname
	\multiply\count255 by 256\advance\count255 by #3
	\multiply\count255 by 16
	\advance\count255 by \csname#4fam\endcsname
	\multiply\count255 by 256\advance\count255 by #5
	\expandafter\delcode\expandafter`\csname#1\endcsname=\count255
	\symbol@mark{#1}{8}}%
%
\def\DeclareMathDelimiter#1{\check@definition{#1}%
	\ifcat\noexpand#1\relax
	\def\Large@stuff{\noexpand\delimiter}%
	\expandafter\@DeclareMathDelimiter
	\else\expandafter\@xDeclareMathDelimiter\fi#1}%
%
\def\DeclareMathRadical#1#2#3#4#5{%\check@definition{#1}%
	\edef#1{\noexpand\radical\noexpand"%
	\expandafter\hexnumber@\csname#2fam\endcsname\gobble@quotes#3%
	\expandafter\hexnumber@\csname#4fam\endcsname\gobble@quotes#5 }%
	\symbol@mark{#1{}}{8}}%
%
\def\DeclareMathAccent#1#2#3#4{%\check@definition{#1}%
        \edef#1{\noexpand\mathaccent\noexpand"%
	\expandafter\hexnumber@\csname#3fam\endcsname\gobble@quotes#4 }%
	\symbol@mark{#1{}}{8}}%
%
% loading math fonts
%
\font\twelvematha=matha10 at 12pt
\font\tenmatha=matha10  \font\ninematha=matha9
\font\eightmatha=matha8 \font\sevenmatha=matha7
\font\sixmatha=matha6   \font\fivematha=matha5
\newfam\mathafam
\font\twelvemathb=mathb10 at 12pt
\font\tenmathb=mathb10  \font\ninemathb=mathb9
\font\eightmathb=mathb8 \font\sevenmathb=mathb7
\font\sixmathb=mathb6   \font\fivemathb=mathb5
\newfam\mathbfam
\font\tenmathx=mathx10
\newfam\mathxfam
%\chardef\mathxfam=4
%\let\tenex=\tenmathx
%
% Initialization
% (make changes in your own file if you want different sizes)
%
\textfont\mathafam=\tenmatha  \scriptfont\mathafam=\sevenmatha
\scriptscriptfont\mathafam=\fivematha
\textfont\mathbfam=\tenmathb  \scriptfont\mathbfam=\sevenmathb
\scriptscriptfont\mathbfam=\fivemathb
\textfont\mathxfam=\tenmathx  \scriptfont\mathxfam=\tenmathx
\scriptscriptfont\mathxfam=\tenmathx
%\def\dagesh#1{{\fam\mathbfam#1}}%
\def\mathafont{\fam\mathafam\tenmatha}%
\def\mathbfont{\fam\mathbfam\tenmathb}%
\let\mathabx@matha=\relax
\let\mathabx@mathb=\relax
\let\mathabx@mathx=\relax
\let\end@mathabx=\relax
\input mathabx.dcl
\catcode`@=12
\let\proofmode=\undefined
\endinput



